Refactoring for Dockerfile Quality: A Dive into Developer Practices and Automation Potential

Docker, the industry standard for packaging and deploying applications, leverages Infrastructure as Code (IaC) principles to facilitate the creation of images through Dockerfiles. However, maintaining Dockerfiles presents significant challenges. Refactoring, in particular, is often a manual and complex process. This paper explores the utility and practicality of automating Dockerfile refactoring using 600 Dockerfiles from 358 open-source projects. Our study reveals that Dockerfile image size and build duration tend to increase as projects evolve, with developers often postponing refactoring efforts until later stages in the development cycle. This trend motivates the automation of refactoring. To achieve this, we leverage In Context Learning (ICL) along with a score-based demonstration selection strategy. Our approach leads to an average reduction of 32% in image size and a 6% decrease in build duration, with improvements in understandability and maintainability observed in 77% and 91% of cases, respectively. Additionally, our analysis shows that automated refactoring reduces Dockerfile image size by 2x compared to manual refactoring and 10x compared to smell-fixing tools like PARFUM. This work establishes a foundation for automating Dockerfile refactoring, indicating that such automation could become a standard practice within CI/CD pipelines to enhance Dockerfile quality throughout every step of the software development lifecycle.

==> 03-relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

\subsection{Docker-based projects Quality Evaluation}

Docker's documentation offers best practicess\footnote{\url{https://docs.docker.com/develop/develop-images/dockerfile_best-practices}} for addressing Dockerfile smells. However, developers adherence to these guidelines is inconsistent. These smells, akin to traditional configuration code smells \cite{ushar2016does}, indicate design flaws that, although not bugs, negatively affect Docker images.

In \cite{yiwen2020characterizing}, authors have categorized Dockerfile smells into two primary types: \textit{DL}-smells, which breach Docker's official best practices, and \textit{SC}-smells, which violate basic shell script conventions. Their empirical study revealed that most open-source projects exhibited Dockerfile smells, with \textit{DL}-smells occurring more frequently than \textit{SC}-smells. Similarly, Durieux et al. \cite{durieux2024empirical} have investigated how shell smells in Dockerfiles increase image size, affecting distribution efficiency and scalability.

In this context, Hadolint\footnote{\url{https://github.com/hadolint/hadolint}} and ShellCheck\footnote{\url{https://github.com/koalaman/shellcheck}} are examples of tools developed to lint Dockerfiles and Bash code within RUN instructions, identifying \textit{SC}-smells.

Henkel et al. \cite{jordan2020learning} have developed Binnacle to mine Bash-related from over 178,000 Dockerfiles. Xu et al. \cite{iwei2019dockerfile} have introduced \textit{TF}-smells, showing how the risky practice of leaving temporary files in Docker images during the build process can inflate image size and complicate distribution.

Beyond detection, some studies have explored the automation of Dockerfile smell repairs. For example, \textit{Parfum} \cite{durieux2023parfum} detects and automatically repairs Dockerfile smells, evaluating repair effectiveness in terms of build failure and image size. Furthermore, Rosa et al.\cite{rosa2024not} have evaluated Hadolint writing practices by experts and ranked 26 additional Dockerfile smells, offering guidance for high-quality Dockerfile writing.


Other studies, such as \cite{wu2020exploring} used linear regression to analyze Dockerfile quality and project characteristics, revealing statistical correlations.  Cito et al. \cite{Cito2017MSR} found that missing version pinning in Dockerfiles often causes build issues, leading to non-reproducible builds. In \cite{henkel2021shipwright}, a human-in-the-loop system using a modified BERT model, has been devoloped for repairing Dockerfiles, showing potential for automating repairs and boosting build success. Most studies target Bash issues in the RUN instruction. However, Dockerfiles involve various instructions and stages, all addressed in our work.

Tackling Dockerfile smells is critical as they often indicate technical debts in Docker projects, such as large images leading to slower deployments and higher resource usage, requiring refactorings to enhance performance ~\cite{ksontini2021refactorings}.

In \cite{ksontini2024drminer}, DRMiner has been introduced for identifying and analyzing Dockerfile refactorings, providing semantics-aware static analysis. Although this tool indicates future potential for automated Dockerfile refactoring, to the best of our knowledge, no tool currently achieves full automation. Similarly, ~\cite{rosa2022assessing} have suggested methods to improve Dockerfile quality and automate the generation of high-quality Dockerfiles. These studies shift focus from detecting smells to addressing issues through potential automation, enhancing Dockerfile quality. 

In this paper, we fully automate detection and refactoring of Dockerfiles to reduce technical debt and improve their quality.


\subsection{Refactoring Recommendation and Automation}
\textcolor{purple}{Several research efforts have aimed to assist or automate code refactoring using various techniques. Despite the availability of automated tools, studies reveal that refactoring is often performed manually due to issues like tool integration and lack of support for real-world scenarios \cite{eilertsen2020refactoring}.}


\textcolor{purple}{ML techniques have been extensively adopted for recommending refactorings in source code. Nyamawe et al. \cite{nyamawe2020feature} suggested refactorings based on the history of previously applied refactorings, requested features, and detected code smells. They utilized classifiers such as LR, CNN, MNB DT, RF, and SVM. Sagar et al. \cite{Sagar2021} explored 800 open-source Java projects, identifying 5004 commits suitable for refactoring to create a balanced dataset of five types of refactorings, using RF, SVM, and LR for identification.}
\textcolor{blue}{The advent of Large Language Models (LLMs) has significantly influenced the field of software development, showing great promise in automating the refactoring process. Zhang et al. \cite{zhang2024refactoring} demonstrated the ability of LLMs to be fine-tuned for specific programming tasks like code completion and bug fixing, crucial for software maintenance and improvement. Their work highlights the potential of LLMs in automated program repair, outperforming traditional methods by learning from vast amounts of code examples. In \cite{white2023chatgpt}, White et al. have presented a catalog of prompt patterns for software engineering activities using ChatGPT (Chat Generative Pre-trained Transformer), including six prompt patterns for code refactoring tasks such as enforcing certain coding principles. Madaan et al. \cite{madaan2023selfrefine} employed Codex, a type of LLM, for improving the readability of variable names and comments through iterative program refinement based on feedback generated by Codex, a method termed Self-Refine. Shirafuji et al.\cite{shirafuji2023refactoring} demonstrated the use of GPT-3.5 to suggest less complex versions of Python programs. The model, when prompted with few-shot examples, was able to refactor 95.68\% of programs effectively, reducing the average cyclomatic complexity by 17.35\% and the number of lines by 25.84\%.}
\textcolor{blue}{In addition to traditional refactoring capabilities, recent studies have highlighted the potential of in-context learning in enhancing the performance of LLMs in software engineering tasks \cite{incontext2024}. The concept of in-context learning allows models to adapt to new tasks without extensive retraining, using few-shot learning techniques. This approach has shown significant improvements in the ability of LLMs to understand and refactor complex code snippets by providing relevant examples within the immediate context of the task.}
\textcolor{blue}{While significant advancements have been made in source code refactoring, there exists a noticeable gap in tools specifically designed for IaC, particularly for Docker. Leveraging LLMs could provide a pioneering approach to automating and recommending Docker-specific refactorings. In this context, Srivatsa et al. \cite{srivatsa2024survey} have highlighted the potential of LLMs in generating IaC configurations. By leveraging the code-generation capabilities of LLMs, the process of creating IaC configurations could be automated, making it more accessible to developers who may not have specialized skills in IaC.}
\textcolor{blue}{To the best of our knowledge, there has been \textbf{no} comprehensive study assessing the application of LLMs specifically for Docker refactoring. Our research compares the effectiveness of Dockerfile refactoring using LLMs with that of developers while maintaining project behaviors. We deeply examine the reasons for build failures with both developers and LLMs, providing insights into the challenges and potential solutions for automating Dockerfile refactoring.}


==> 06-discussion.tex <==
\section{Discussion and Implications}
\label{sec:discussion}

\begin{itemize}
     \item talk about the relation between RQ1 and RQ2
     \item talk about commit checkout. so that changes to the size of the app doesn't make any issues
\end{itemize}



==> approach_copy.tex <==
\subsection{Refactoring Demonstration Retrieval}

In RQ2, we use technical debts defined in \cite{ksontini2021refactorings} to develop a score-based demonstration selection strategy. We focus on image size, build duration, maintainability, and understandability to score the train set. 

As illustrated in \autoref{fig:apprach}. Given a test Dockerfile $V_{Before\_Test}$, we identify the most relevant dockerfile refactoring demonstrations \( RD_i \) using the following formula: 
%\vspace{-3mm}
\begin{equation}
\setlength{\arraycolsep}{1pt}
\renewcommand{\arraystretch}{0.8}
\scalebox{0.9}{ % Adjust scaling factor as needed
  \fbox{
    \begin{minipage}{0.9\linewidth}
      \small
      \begin{align*}
      \text{score}(RD_i) = & \, 0.2 \times \text{Textual\_similarity}(V_{\text{Before}_i}, V_{\text{Before}\_Test}) + \\
                           & \, 0.2 \times \text{understandability\_score}(V_{\text{Before}_i},V_{\text{After}_i}) + \\
                           & \, 0.2 \times \text{maintainability\_score}(V_{\text{Before}_i}, V_{\text{After}_i}) + \\
                           & \, 0.2 \times \text{image\_size\_score}(V_{\text{Before}_i}, V_{\text{After}_i}) + \\
                           & \, 0.2 \times \text{build\_duration\_score}(V_{\text{Before}_i},V_{\text{After}_i})
      \end{align*}
    \end{minipage}
  }}
\end{equation}
The components of the score are defined as follows:

\begin{itemize}
    \item \textbf{Textual\_similarity}: Calculated using BM-25 \cite{robertson1995okapi}.
    \item \textbf{Understandability (or Maintainability) score}: Assigned a value of 1 if the understandability (or maintainability) of \( V_{\text{After}_i} \) is greater than \( V_{\text{Before}_i} \), 0 if they are the same, and -1 if it is worse.
    \item \textbf{Build time (or image size) score}: Calculated as  \( 1 - \frac{\text{build\_duration}(\text{or  image\_size) }(V_{\text{After}_i})}{\text{build\_duration} ( \text{or  image\_size)}(V_{\text{Before}_i})} \), quantifying the improvement in build duration  (or image size).
%\textbf{Image size score}: Calculated as \( 1 - \frac{\text{image\_size}(V_{\text{After}_i})}{\text{image\_size}(V_{\text{Before}_i})} \), quantifying the improvement in image size.
\end{itemize}

For each query, we compute the score over the entire corpus of demonstrations, rank the train corpus based on this score, and select the top $n$ based on the number of shots. For instance, we select the top example for one-shot, the top 20 examples for 20-shot, and so on. When adding the demonstrations to the prompt, we order them in ascending order, meaning the one with the highest score will be closest to the query Dockerfile. This ordering follows the findings by Gao et al. \cite{gao2023makes}.

This approach returns demonstrations that closely match the query Dockerfile and exhibit the greatest overall quality improvements. By focusing on content similarity, we ensure that the model understands the specific needs of different Dockerfiles, which can differ in terms of applications and commands. Moreover, prioritizing quality improvements enables the model to learn optimal practices from the best examples.

We automatically compute the image size, in megabytes (MB), and build duration, in seconds (s), using an automated script. For maintainability, understandability, and Dockerfile behavior, we employ a manual assessment. The assessment is performed by three authors of the paper.


\subsection{Evaluation metrics}

To evaluate the performance of LLMs in automating Dockerfile refactoring, as shown in \figure{}, we conduct automated builds and measure build failure rates. Dockerfiles that fail to build are excluded from further analysis; we simply record these as failures and retain a copy of the failure log for future reference. We also perform behavioral assessments to ensure that the refactoring automation does not alter the expected behavior of the Dockerfiles, excluding any that do.

We calculate metrics related to technical debt \cite{ksontini2021refactorings} for the test set (including original and manually refactored dockerfiles) and for the output of the LLM. These metrics include image size and build time, which are quantitatively measured. For maintainability and understandability, we employ the same scoring system as used in \autoref{}.

Manual assessment of understanbility, maintainability and behavior of the test dataset and the output of llm is conducted by six active industry developers, each with an average of three years of Docker experience, participate in this assessment through an industry-sponsored collaboration. To ensure unbiased results, they are kept unaware of which Dockerfile version is refactored. Both original and refactored Dockerfiles (from LLM or developers) are presented for evaluation. 

Developers complete a pre-study survey collecting background information such as programming experience and their role within their companies. To minimize potential bias, we provide participants with a two-hour lecture on Docker quality assessment and refactoring, covering general refactoring knowledge and specific interpretation of Dockerfile practices.

%Each developer completes a pre-study survey collecting background information such as programming experience and their role within their companies. To minimize potential bias, we provide participants with a two-hour lecture on Docker quality assessment and refactoring, covering general refactoring knowledge and specific interpretation of Dockerfile practices.

%We can make this shorter
\textcolor{purple}{In order to annotate the results within the dataset, we follow the Kappa cross-validation process. During this validation, each participant is assigned an average of 297 Dockerfiles, ensuring each Dockerfile is evaluated by three developers. The value of an assessment (whether behavior, maintainability, or understandability) is considered only if at least two evaluators agree, with an overall Cohen’s kappa of \textcolor{red}{0.84}. Detailed information about the participants and the Dockerfiles they evaluated can be found in our replication package \cite{ICSE25_replication}.}

==> intro_draft.tex <==
\section{Introduction}
\label{introduction}

% IaC and transition to containarisations
%In recent years, Infrastructure as Code (IaC) has transformed software infrastructure management by allowing developers to define configurations through code, enhancing consistency and reducing configuration drift \textbackslash{}cite\{guerriero2019adoption, sokolowski2022infrastructure\}. A key aspect of IaC is containerization, which packages applications and their dependencies into lightweight, self-contained units \textbackslash{}cite\{debab2021containers\}.


%In recent years, the paradigm of IaC has revolutionized the way software infrastructure is managed and deployed. It has enabled developers to define infrastructure configurations through code. 
%This approach has been widely adopted in modern DevOps practices, as it helps maintain consistency across environments and minimizes the risk of configuration drift 

%\textcolor{purple}{Recently, IaC has transformed software infrastructure management and deployment by allowing developers to define infrastructure configurations through code, thereby maintaining consistency across environments and minimizing the risk of configuration drift in modern DevOps practices \cite{guerriero2019adoption, sokolowski2022infrastructure}. Central to IaC is containerization, which encapsulates applications and their dependencies into lightweight, self-contained units known as containers \cite{debab2021containers}. 


Docker has emerged as the de facto industry standard, offering a platform for creating, deploying, and managing these units \cite{bullington2020docker}. The contents of a Docker container are defined by Dockerfile declarations, which specify the instructions and their execution order. Often found in source code repositories, these files facilitate the building of images that can then be run as containers, thereby bringing the hosted software to life in its execution environment \cite{miell2019docker}.


%Docker has become the industry standard for creating, deploying, and managing containers.  The contents of a Docker container are defined by Dockerfile declarations, which specify the instructions and their execution order. Often found in source code repositories, Dockerfiles facilitate building images that can then be run as containers, thereby bringing the hosted software to life in its execution environment
%Docker has become the industry standard for creating, deploying, and managing containers, with Dockerfile declarations defining their contents  and specifying the instructions and their execution order \cite{bullington2020docker}. Often found in source code repositories, Dockerfiles facilitate building images that can then be run as containers, thereby bringing the hosted software to life in its execution environment \cite{miell2019docker}. 
%Dockerfiles facilitate the building of images that can then be run as containers, 


%Docker has emerged as the de facto industry standard, offering a platform for creating, deploying, and managing these units \cite{bullington2020docker}. The contents of a Docker container are defined by Dockerfile declarations, 
%Often found in source code repositories, these files enable the creation of images for container execution,

%Despite being the backbone of containerization, Dockerfiles are often plagued with problems such as smells \cite{durieux2024empirical}, anti-patterns \rania{cite}, and vulnerabilities \cite{}. In the case of smells, several works have been proposed to detect and fix them 

% problem statment
Despite being the backbone of containerization, Dockerfiles are often plagued with problems such as smells \cite{durieux2024empirical}. In this context, several works have been proposed to detect and fix them \cite{yiwen2020characterizing, bui2023dockercleaner, durieux2023parfum}. However, most solutions focus on bash commands, which are typically embedded within specific instructions in Dockerfiles, mainly the RUN instruction. Common bash smells include the installation of unnecessary packages and missing version pinning \cite{yiwen2020characterizing,rosa2024not}. While bash-based solutions are useful, they fall short of addressing the broader structure of Dockerfiles, which are not limited to the RUN instruction. Instead, Dockerfiles include various instructions and stages that together form the final image.
%Dockerfiles consist of a combination of various instructions and could be composed of multiple stages that together form the final image. }
%Most solutions focus on bash commands within Dockerfile instructions, especially RUN, often . 
% challenges impacting quality metrics




Developers face challenges beyond managing shell scripts in Dockerfiles, such as optimizing instructions and defining the right stages to ensure overall quality. A key challenge is maintaining small \textbf{image sizes}. Each instruction within a Dockerfile adds a layer to the final image, potentially leading to bloated containers if not managed carefully. Choosing the appropriate base image and effectively utilizing multi-stage builds can mitigate this issue, but achieving the right balance requires considerable expertise and effort \cite{straesser2023empirical, durieux2024empirical}.
\textbf{Maintaining} Dockerfiles is another challenge, with common bugs and unexpected behaviors often arising, especially when the base image tag is not specified correctly. Additionally, some developers, unaware of the availability of official and trusted images, manually add dependencies, which can lead to inconsistencies and complicate future updates \cite{azuma2022empirical}. \textbf{Build duration} is influenced by several factors, including the order of instructions, the complexity of multi-step commands, and the number of instructions. Poorly optimized sequences and complex instructions can lead to high build durations and incur high costs, complicating the workflow \cite{wu2022understanding}. 
As a project progresses through its development stages, the content of the Dockerfile may be revised many times \cite{9359307}, which can affect \textbf{understandability} and complicate subsequent updates.


% Frequent modifications to Dockerfiles can affect \textbf{understandability}, making them harder to maintain. As a project progresses through its development stages, the content of the Dockerfile may be revised many times \cite{9359307}, further complicating maintenance. Fixing Dockerfile issues often takes more time than addressing source code problems.


%Fixing Dockerfile issues often takes more time than addressing source code problems \cite{Yiwen2020}.}

%By eliminating technical debts related to maintainability, understandability, build duration, and image size, refactoring enhances the reliability and longevity of containerized applications. This process addresses common issues like high number of layers, large base images, and improper instruction ordering, ultimately improving the overall Dockerfile quality \cite{ksontini2021refactorings}.

% transition from manual to automation specific for Docker then 

% transition to refactoring definition
To address these challenges and improve the overall quality of Dockerfiles \cite{ksontini2021refactorings}, the predominant method has been manual refactoring. This approach depends heavily on developers' expertise to enhance the internal structure of the code without changing its external behavior, as no automated tools are currently available for this purpose. Despite its potential effectiveness, this manual method is notably more time-consuming than resolving source code issues \cite{Yiwen2020} and is inherently prone to human error.

%To address these challenges and improve the overall Dockerfile quality \cite{ksontini2021refactorings},  \textbf{manual refactoring of Dockerfiles} has been predominantly employed. It consists of relying primarily on developers' efforts to improve the internal structure of the code without altering its external behavior, thereby mitigating risks associated with poor quality.  This method is even more time-consuming than addressing source code problems \cite{Yiwen2020} and error-prone due to the lack of automated tools.

%Despite the existance of refactoring tools designed for languages like Java, Python and C, they remain unsuitable for Dockerfiles due to their unique IaC nature and declarative syntax.



%Dockerfiles, hosting applications in various languages (e.g., Java, PHP, Go), and domains (e.g., ML, Web), require substantial modifications and expertise beyond basic instruction or stage changes.
%Multi-stage building adds further complexity with base image selection, command management, and file transfer, making search-based methods and traditional ML impractical due to the need for extensive datasets and deep learning.

%Dockerfiles are versatile, supporting applications across various programming languages (e.g., Java, PHP, Go) and domains (e.g., machine learning, web development). Refactoring Dockerfiles demands substantial expertise beyond basic modifications, such as selecting appropriate base images, tags, and adjusting dependencies. The process becomes even more complex with extract stage refactoring, which requires determining the optimal number of stages, instructions, and managing file transfers between stages.

Current refactoring tools designed for languages like Java, JavaScript, C, and Python \cite{} are inadequate for Dockerfiles due to the distinct nature of Infrastructure as Code (IaC) and their declarative syntax. Dockerfiles, re used to containerize applications across various programming languages (e.g., Java, PHP, Go) and domains (e.g., machine learning, web development). Refactoring Dockerfiles involves more than simple structural changes and requires expertise in selecting appropriate base images, tags, and adjusting dependencies. Techniques such as Extract Stage refactoring add further complexity by necessitating decisions on the optimal number of stages and the selection of files to transfer between them. Consequently, automating Dockerfile refactoring with traditional machine learning or search-based methods is impractical.

%Dockerfiles, which can host applications across various (e.g., Java, PHP, Go) and domain (e.g., ML, Web), require substantial modifications and deep expertise that go beyond simple changes to instructions or stages. Multi-stage building adds further complexity, involving base image selection, command and variable management, and data transfer between stages, making search-based methods and traditional machine learning impractical due to the need for extensive datasets and deep learning.

%Recently, Large Language Models (LLMs) have proven to be valuable for various software engineering tasks, including code completion \cite{ciniselli2021empirical}, code summarization \cite{feng2020codebert}, commit message generation \cite{eliseeva2023commit}, code transformation \cite{dilhara2024unprecedented, ramos2023melt}, and bug report reproduction \cite{feng2024prompting}. Due to their training on vast code repositories that include billions of Dockerfiles authored by real developers, we theorize that LLMs can effectively mimic human behavior in writing Dockerfiles, making them capable of suggesting accurate and high-quality refactorings.

Over the past few years, LLMs have proven to be valuable in software engineering tasks like code completion\cite{ciniselli2021empirical}, code summarization \cite{feng2020codebert}, commit message generation \cite{eliseeva2023commit}, code transformation \cite{dilhara2024unprecedented}\cite{ramos2023melt}, and bug report reproduction \cite{feng2024prompting}.  
Given their training on vast code repositories, including billions of Dockerfiles created by real developers,  we theorize that LLMs can effectively mimic human behavior in writing Dockerfiles and suggest accurate, high-quality refactorings.

%Given their training on vast code repositories, including billions of Dockerfiles authored by real developers,  we theorize that LLMs can effectively mimic human behavior in writing Dockerfiles, making them capable of suggesting accurate and high-quality refactorings.

By bridging the gap between LLM capabilities and the complexity of Dockerfile refactorings, we present in this paper a novel study assessing the application of LLMs for automating Dockerfile refactoring. Our research incorporates in-context learning and yields several significant findings:

\begin{itemize} 
\faKey\ F1: Despite their potential for automating Dockerfile refactoring, LLMs are currently constrained by a narrow range of refactoring types. For instance, when prompted, \textit{GPT-4o} applied only two types of refactorings, whereas developers used ten. Thus, incorporating in-context learning with diverse examples can significantly enhance performance, leading to notable improvements in Docker image size and build duration as projects mature. 
\end{itemize}
\begin{itemize}
\faKey\ F2: Our study indicates that a significant proportion of Dockerfiles undergo their first refactoring during the mid to later stages of development, with refactoring actions comprising over half of the commits during this period. This highlights the importance of automating refactoring to address these late-stage updates efficiently. 
\end{itemize}
\begin{itemize}
\faKey\ F3: Our comparison shows that LLMs significantly outperform manual refactoring, especially in reducing image size, with more refactoring demonstrations further enhancing their performance. However, this comes with a minor trade-off in understandability and maintainability. 
\end{itemize}
\begin{itemize}
\faKey\ F4: Build failures in Dockerfile refactorings, primarily due to build context and dependency issues, closely match in frequency between manual and automated methods. 
\end{itemize}

%F3: Our comparison reveals that LLMs significantly outperform manual refactoring, especially in reducing image size, with increased refactoring demonstrations further enhancing LLM performance. Nevertheless, this improvement comes with a minor trade-off in understandability and maintainability. 




%Our study shows that LLMs have the potential to be applied effectively to Dockerfile refactoring. 




==> trash_old_02-introduction.tex <==
\section{Introduction}
\label{introduction}


Containerization is a software development approach aimed at packaging an application together with all its dependencies and execution environment in a light-weight, self-contained unit, of which Docker has become the de-facto industry standard. The contents of a Docker container are defined by declarations in the Dockerfile, which specify the Docker instructions and the order of their execution, following the notion of Infrastructure-as-Code (IaC) 


\emna{ incorporate sth related to build and containers here }. They can often be found in source code repositories and enable the hosted software to come to life in its execution environment.  Dockerfiles, being the backbone of containerization, are crucial, yet they are often plagued with problems such as smells, anti-patterns, and vulnerabilities, leading to compromised maintainability, increased resource consumption, long build times, and reduced performance \emna{add some stats here}. 
It is essential to address these issues, and this is where the significance of refactoring Dockerfiles comes into play. It involves improving the internal structure of a Dockerfile without altering its external behavior. This is essential for mitigating risks associated with poor quality Dockerfiles, ensuring the reliability and longevity of containerized applications by resolving issues like high number of layers, big base images, and improper instruction ordering.
These refactorings are done fully manually by developers, due to the absence of automated tool.

Each refactoring operation in Dockerfile aﬀects one or multiple instructions and sometimes can lead to the remove or addion of stages, depending on the refactoring type. Developers usually perform more than one refactoring tactics at single commit.


each change, big or small in Dockerfile, is a risk for bugs and issues \cite{tanaka2023meta} 
Despite the original intention of improving software quality and productivity through refactoring, manual application of refactoring edits often leads to error-proneness and can introduce unexpected behaviors in Docker containers, potentially compromising the application's functionality, security, and maintainability.

\emna{why automation of refactoring is important}. 

While several refactoring autommation tools exist, catering predominantly to Java, with some extending to JavaScript, C, and Python \cite{}, they are not suitable for Dockerfiles. This is due to Dockerfiles' unique Infrastructure as Code (IaC) nature and declarative syntax, which significantly differ from traditional source code.  Additionally, the types of refactorings in Dockerfiles are distinct, further necessitating specialized tools for their detection and analysis. 


\emna{explain why tradional machine learning or seach based methods cannot be used to automate refactoring in dockerfile give explicit example and why LLMs are the best option}

Recently, Large Language Models (LLMs) [24, 29, 46] are emerging as powerful companions
for software engineering tasks: code completion [15], code summarization [24], commit message
generation [2], code transformation [19, 49], reproducing bug reports [54], etc. Given LLMs’ training
on extensive code repositories that contain billions of methods written by actual developers, we
hypothesize that they are more likely to imitate human behavior by mimicking how developers
form functions, thus are likely to suggest refactorings that developers would accept.

Recently, in-context learning has been shown to be an effec-
tive way to exploit the domain knowledge hidden in the LLMs

[8, 11, 48, 60], since the format of the inputs to the model can
be consistent to that during the pre-training process. Inspired by
these studies, we aim to investigate the feasibility of addressing

the multi-intent comment generation task with in-context learn-
ing. Generally, in-context learning requires to provide a prompt

to the model which is composed of a natural language instruction

describing the detailed information of the task, (optionally) a hand-
ful of examples demonstrating how the task could be well done,

and a query that is required to be addressed. Therefore, a follow-
up question is that, with in-context learning, how can we obtain

better results from the LLMs (e.g., if it is possible by designing
prompts that can guide the LLMs towards the desired output).


To bridge this void, we introduce ..., a tool tailored for automation of Dockerfile-specific refactoring using In-context learning.









The remainder of this paper is organized as follows: in the next section, we summarize several related works. We describe the proposed tool in \ref{sec:04-Approach}. In \ref{sec:05-Evaluation}, we present the results of our quantitative analysis regarding the correctness and generalization of DRMiner as well as our qualitative analysis on the misdetected refactorings. Section \ref{sec:07-threats} reports the threats to validity. We end up with a conclusion and discuss our perspectives in \ref{sec:conclusion}.


\textbf{Replication Package.} DRMiner tool and all materials used in our study are available in our replication package~\cite{appendix}.

%The rest of the paper is structured as follows: Section 2
%provides an overview of the study with a goal and corresponding research questions. Section 3 describes a catalog
%containing implementation and design configuration smells.
%Section 4 details the developed tool, mining Puppet repositories from GitHub and applying the tool on the repositories. Section 5 provides detailed answers to the research
%questions. We discuss related work in Section 6.


%This paper embarks on a journey, chronicling the inception, realization, and assessment of DRMiner. Our endeavor seeks to augment the academic conversation on Dockerfile refactoring and furnish the developer community with a robust suite of tools.


%The remainder of this paper is structured as follows: section 2 presents 

%Exisiting approaches conducted in diverse domains, including Object-Oriented Programming and Web Services, emphasize the significance of understanding developers' refactoring choices and the underlying motivations driving those choices. \cite{antoniol2004automatic,bavota2012refactoring,bavota2015quality,kim2011api,palomba2017relationship,rachatasumrit2012impact,weissgerber2006error}. These insights illuminate the evolutionary trajectory of the source code, refining review methodologies and enhancing overall comprehension of the codebase. Within containerization and Docker, a similar need arises for comprehending Docker quality issues and exploring Docker-specific refactorings and refactoring detection tools.




%identifying refactoring benefits
%detecting



\begin{comment}
each change, big or small in Dockerfile, is a risk for bugs and issues \cite{tanaka2023meta} missteps or inaccuracies during the refactoring process can introduce unexpected behaviors in Docker containers, potentially compromising the application's functionality, security and maintainability. By detecting these potential sources of errors early, developers can preemptively address issues before they escalate.In this case, the maintainers have to make the identical changes to those multiple
Dockerfiles. Several studies focus on the quality of Dockerfile. Wu
et al. \cite{10.1145/3379597.3387483} found that up to 85.2\% of Docker projects have at least one broken build. They also found that the more frequently developers build projects, the less likely projects fail to build, while the
more often developers fail to build, the longer it takes to fix issues.

(2)
 ..... (2) ..... and (3) ...


\textbf{Detecting Potential Error Sources:} Missteps or inaccuracies during the refactoring process can introduce unexpected behaviors in Docker containers, potentially compromising the application's functionality, security and maintainability. By detecting these potential sources of errors early, developers can preemptively address issues before they escalate. 
Each change, big or small in Dockerfile, is a risk for bugs and issues \cite{tanaka2023meta}






\textbf{Capturing Intent of Changes and Replaying:} Refactorings are not arbitrary; specific needs or objectives drive them. Grasping the underlying rationale behind these changes is crucial. This understanding aids developers in ensuring that the refactoring aligns with the intended purpose and doesn't inadvertently introduce new issues. This comprehension is equally invaluable for code reviewers, providing essential context that makes the review process more effective leading to more informed decisions. 
In the dynamic world of software development, where multiple iterations and versions exist, the ability to accurately reproduce manual refactorings becomes indispensable. This ensures that Docker configurations remain consistent across different deployments, fostering reliability and predictability in application behavior.  
Projects that frequently change Dockerfile and modify more lines tend to be more successful (higher forks) \cite{9359307}
\textbf{Relation to Other Changes:} Refactorings often don't exist in isolation. They can trigger or be influenced by changes in related code or configuration. Being aware of refactoring practices and their interrelations can empower developers to anticipate and address cascading changes, ensuring that the entire ecosystem remains harmonized. 
Dockerfiles are coupled tightly with other files.
Those co-changed revisions account for more than 70\% of all revisions \cite{9359307}

\textbf{Relation to Software Metrics:} Refactorings, while primarily aimed at improving code structure or addressing specific issues, can also have a broader impact on software metrics. By analyzing the repercussions of refactorings on metrics like build time, image size, container performance, resource efficiency, and response times, stakeholders can derive actionable insights. This not only aids in optimizing the current setup but also provides valuable feedback for future refactoring endeavors. 
\\
\end{comment}
%Empirical studies spanning domains like Object-Oriented Programming and Web Services accentuate the importance of deciphering developers' refactoring choices and the motivations behind them \cite{antoniol2004automatic,bavota2012refactoring,bavota2015quality,kim2011api,palomba2017relationship,rachatasumrit2012impact,weissgerber2006error}. These insights illuminate the evolutionary trajectory of the source code, refining review methodologies and enhancing overall comprehension of the codebase. \am{i think this is out of scope, you can just mention this in related work or in the beginning of the introduction}
%This becomes even more pertinent given the absence of automated refactoring tools for Docker, highlighting the reliance on manual refactoring practices. 

%Identifying refactoring within the Docker ecosystem is both paramount and intricate. Developers often inadvertently overlook the documentation of their refactoring activities, frequently merging them with other modifications. This gap highlights an urgent need—a comprehensive tool capable of adeptly discerning Dockerfile refactoring intricacies. 



%the unique challenges posed by Docker necessitate specialized solutions.


%\textcolor{blue}{To the best of our knowledge, there is \textbf{no} previous work done to fill this gap} and that which ...



==> trash_old_02-introduction_update.tex <==
\section{Introduction}
\label{introduction}
In recent years, the paradigm of Infrastructure as Code (IaC) has revolutionized the way software infrastructure is managed and deployed. IaC enables developers to define infrastructure configurations through code. This approach is widely adopted in modern DevOps practices, as it helps maintain consistency across environments and minimizes the risk of configuration drift \cite{guerriero2019adoption, sokolowski2022infrastructure}. Central to IaC is containerization, which encapsulates applications and their dependencies into lightweight, self-contained units, also known as containers \cite{bullington2020docker}. Among the various containerization technologies, Docker has emerged as the de facto industry standard, offering a platform for creating, deploying, and managing these units. The contents of a Docker container are defined by declarations in a Dockerfile, which specify the instructions and their execution order. These files, often found in source code repositories, facilitate the building of images that can then be run as containers, bringing the hosted software to life in its execution environment \cite{}. 

% problem statment
Dockerfiles, being the backbone of containerization, are crucial, yet they are often plagued with problems such as smells \cite{durieux2024empirical}, anti-patterns, and vulnerabilities. 
Several works have been proposed to detect and fix these smells \cite{wu2020characterizing, bui2023dockercleaner, durieux2023parfum}. Most of these solutions are focused on bash commands, which are typically embedded within specific instructions in Dockerfiles, mainly the RUN instruction. Common bash smells include the installation of unnecessary packages and missing version pinning \cite{yiwen2020characterizing, rosa2024not}. While these bash-based solutions are useful, they fall short of addressing the broader structure of Dockerfiles. Dockerfiles are not limited to the RUN instruction; they consist of a combination of various instructions and can be composed of multiple stages that together form the final image.

Developers face challenges beyond managing shell scripts within Dockerfiles. They need to create the optimal combination of instructions and define the appropriate stages to achieve the best overall quality of the Dockerfile. Ensuring small \textbf{image sizes} is critical, as each instruction adds a layer, potentially leading to bloated containers if not managed carefully, which can impact the container start time \cite{straesser2023empirical} and tend to have more smells \cite{durieux2024empirical}. 


% expand the four quality issues within docker file
One of the primary struggles developers face is ensuring small \textbf{image sizes}. Each instruction within a Dockerfile adds a layer to the final image, leading to bloated containers if not managed carefully. Selecting the appropriate base image and utilizing multi-staging effectively can mitigate this issue, but finding the right balance requires significant expertise and effort.

\textbf{Maintaining} the Dockerfile itself is another major challenge. Common bugs and unexpected behaviors often arise, especially when the base image tag is not specified correctly. For instance, using a base image without specifying a tag might work initially, but future updates to the base image can introduce incompatibilities, causing the Dockerfile to fail. Additionally, projects often contain multiple Dockerfiles with similar content but different configurations. Any change in one file necessitates changes in all others, highlighting the importance of using ARG instructions to manage shared configurations efficiently.

\textbf{Build time} is heavily influenced by the order of instructions within the Dockerfile. Poorly optimized instruction sequences can lead to significantly longer build times, affecting the overall development workflow. Developers must carefully plan the order of instructions to minimize build times, but this optimization process can be complex and time-consuming.

\textbf{Understandability} is another critical issue. Changes in the application frequently necessitate modifications to the Dockerfile, and as the application evolves, the Dockerfile must be updated accordingly. This frequent modification can make the Dockerfile harder to understand and maintain. Fixing issues within the Dockerfile often takes more time than addressing source code problems due to the complexity of the containerization process and the interdependencies between instructions.


% transition to refactoring definition
It is essential to address these issues, and this is where the significance of refactoring Dockerfiles comes into play. Refactoring involves improving the internal structure of a Dockerfile without altering its external behavior, which is crucial for mitigating risks associated with poor quality Dockerfiles. By focusing on eliminating technical debts related to maintainability, understandability, build time, and image size, refactoring ensures the reliability and longevity of containerized applications. This process addresses common issues such as a high number of layers, large base images, and improper instruction ordering, ultimately enhancing the overall quality and efficiency of Dockerfiles \cite{ksontini2021refactorings}.





% transition from manual to automation specific for Docker
Currently, Dockerfile refactoring is predominantly a \textbf{manual task}, which is time-consuming and error-prone due to the lack of automated tools. Existing refactoring automation tools for languages like Java, JavaScript, C, and Python are not suitable for Dockerfiles due to their unique Infrastructure as Code (IaC) nature and declarative syntax. Refactoring in Dockerfiles is not a simple matter of moving, adding, or deleting instructions or stages; it involves significant modifications that require a deep knowledge base.

% Currently, Dockerfile refactoring is predominantly a \textbf{manual task}, which is time-consuming and error-prone due to the lack of automated tools. While several refactoring autommation tools exist, catering predominantly to Java, with some extending to JavaScript, C, and Python \cite{}, they are not suitable for Dockerfiles. This is due to Dockerfiles' unique Infrastructure as Code (IaC) nature and declarative syntax, which significantly differ from traditional source code.  Additionally, the types of refactorings in Dockerfiles are distinct, further necessitating specialized tools for their automation. 



% When we look at the common approaches for automating refactoring in other domains, we find search-based algorithms and machine learning. Refactoring in Dockerfiles is not a simple matter of moving, adding, or deleting instructions or stages; it involves significant modifications that require a deep knowledge base.

% present the power of LLM
For instance, applying multi-stage building necessitates the choice of correct base images with their correct versioning, additional new commands, new variables, new instructions, and a careful choice of what data to move from one stage to the other. This complexity makes search-based methods impractical, and traditional machine learning would require a vast dataset and significant learning depth. Moreover, Dockerfiles can host any application and are not tied to a specific language (e.g., Java, PHP, Go) or domain (e.g., ML, Web). Each has its unique knowledge and details, further complicating the use of traditional automated refactoring methods.


Recently, Large Language Models (LLMs) have emerged as powerful tools for software engineering tasks such as code completion, code summarization, commit message generation, code transformation, and reproducing bug reports. Given LLMs’ training on extensive code repositories containing billions of Dockerfiles written by actual developers, we hypothesize that they are more likely to imitate human behavior by mimicking how Docker developers write their Dockerfiles, thus suggesting refactorings that are correct and of good quality.


For instance, we prompted the LLM (GPT-4o) on 1500 Dockerfiles and found that the LLM consistently applied only two types of refactorings. However, for the same Dockerfiles, developers applied 10 distinct types of refactorings. This discrepancy highlights that while LLMs have potential, they are not yet fully aware of the variety and complexity of Dockerfile refactorings. This realization led us to consider in-context learning.


In-context learning involves providing the model with specific examples and scenarios during its interactions. By feeding the LLM with more detailed and diverse examples of Dockerfile refactorings, we can enhance its understanding and ability to perform a wider range of refactorings. 




% search based methods 
% when we look at the common approaches for automating refactoring in other domains, we find search based algorithms and machine learning 
% refactoring in Dockerfile is not a simple moving/add/delete of instructions or stages. it involves a major modifications of the different   .... that a needs a huge knowledge base.
% for instance, applying multi-stages building necessitate the choice of correct base images with their correct versioning additional new commands / new variable / new instructions and a careful choice of what data to move from one stage to the other. This makes search based methods not appliable and traditional ML would require a huge dataset and large learning depth.

% especially knowing that a dockerfile can host any application and it is not tight to a specific language (java/ php/ go /etc)or domain (ML / Web/ etc). And imagine here each has its proper knowledge and details.  

% Recently, Large Language Models (LLMs) [24, 29, 46] are emerging as powerful companions for software engineering tasks: code completion [15], code summarization [24], commit message
% generation [2], code transformation [19, 49], reproducing bug reports [54], etc. Given LLMs’ training on extensive code repositories that contain billions of Dockerfile written by actual developers, we hypothesize that they are more likely to imitate human behavior by mimicking how docker developers write their dockerfile, thus are likely to suggest refactorings that are correct and of a good quality.

% For instance, we prompted the LLM (gpt4-o) on 1500 dockerfiles and we found out that the LLM for all these cases was applying only two types of refactorings. However, for the same dockerfiles, developers applied 10 types of refactorings. This made beleive that LLMs are not aware of the different types of dockerfile refactoring and make us think about the in context learning.

% Refactoring Dockerfiles is complex due to dependencies between instructions, where small changes can cause build failures, version mismatches, image size issues, and environment variable misconfigurations. Updating packages or altering instruction order can lead to conflicts, while new base images can bloat the final image. Misconfigured environment variables can cause application failures.



% Given the critical importance of Docker and Dockerfiles in the software development lifecycle, it is essential to address the challenges associated with their maintenance and optimization. Automating the refactoring process can significantly enhance the reliability and security of containerized applications, making it a vital area of research and development in the field of software engineering \cite{}.



% \begin{itemize}
%     \item Objectives and Contributions:

% Outline the main objectives of your research.
% Summarize the key contributions your paper makes to the field of software engineering.

% Research questions and main contribution for ewach one
% \end{itemize}

% This paper presents an in-depth exploration of these advanced refactoring techniques, evaluating their effectiveness through a set of metrics designed to measure technical debt and overall quality improvements. Our approach aims to provide developers with automated tools that not only detect and fix issues but also guide them in creating high-quality Dockerfiles that adhere to best practices and industry standards.







% The quality of Dockerfile is determined by a list of 
% maintainability, understandability 
% \begin{itemize}
%     \item promoting the quality attributes
% \end{itemize}

% \begin{itemize}
%     - related works on smells within docker file ..... BASH however ,,,
%     \cite{wu2020characterizing}
%         Missing Version Pinning ( bash ) : Not specifying a concrete version for dependencies, which was one of the most prevalent issues.
%         ****Use of Latest Tag: Utilizing the 'latest' tag instead of a specific version.***
%         Deprecated Instructions: Using outdated commands that may no longer be best practice.
%         Unnecessary Packages ( bash ): Including packages that are not required for the application to function.
%     \cite{bui2023dockercleaner}
%     DockerCleaner: Automatic Repair of Security Smells in Dockerfiles
%         Using the latest tag: This can lead to unpredictable behavior since the latest tag can change without notice.
%         Missing version pinning: Not specifying a concrete version for dependencies.
%         Hardcoded secrets ( Add ENV ): Including sensitive information directly in the Dockerfile.
%         Deprecated instructions: Using commands that are no longer recommended.
%     \cite{durieux2023parfum}
%     Parfum: Detection and Automatic Repair of Dockerfile Smells
%         Temporary File Smell: This occurs when temporary files are used during the build process but are not properly removed, leading to larger image sizes.
%         Missing Version Pinning: Not specifying a version for dependencies, which can lead to unpredictability if dependencies update to incompatible versions.
%         Use of Latest Tag: Using the 'latest' tag for base images, which can be unreliable since the latest version can change.
%         Deprecated Instructions: Using commands that are no longer recommended or have been superseded by better alternatives.
%         Unnecessary Packages: Including packages that are not required for the application to function, which can bloat the image size.
%         Inefficient Commands: Using commands in a way that is not optimal, leading to larger or less efficient images.


        
%     - this bash is only contained in specific instruction in docker file. MAinly RUN instruction. However, the structure of dockerfile is not limited to this instruction, 
%     we have a combination of different instructions and can be composed of different stages that together form the final image.
%     - Developers are facing issues more than just the bare shell script inside docker / 
%     - they need to make the perfect combinations between these instructions and define the right stages to get the best overall quality of the docker file.
    
%     \item challenges that developers are facing in  docker file
%     - they struggle to maintain small containers size / small image size ; however, each instruction within the dockerfile, add layer. 
%     - Developers usually struuglke to find the appropriate base image with the right multi staging
%     - Maintanability: 
%         - Usually within a docker file related to common bugs.
%         - unexpected behaviour: for example base image when not specifying the right tag. It may work now, but in the future when the new version of the base image is uploaded it may fail to work.
%         - Copy of the dockerfile: many dockerfile with the same conetent can be inside the same project but with different configuration --- a change cin one file means a change in every file -- importance of ARG.
%     Build time
%         -- choice of the order of instructions ... can hugely affect the build time 
%     Undersanbvility:
%     - a change in the app can leas to change dockerfile ... content of dockerfile is modifefd frequently in lyficyle of app .. understanble ... fixing issue within docker file takes more time than fixing code source 3adi\\\
        
% \end{itemize}


% \begin{itemize}
%     \item Problem Statement:

% Explain the common issues developers face when working with Dockerfiles, such as technical debts, smells, and vulnerabilities.
% Discuss the manual nature of current refactoring processes and the associated challenges.
% \end{itemize}


% Dockerfiles, being the backbone of containerization, are crucial, yet they are often plagued with problems such as smells \cite{yiwen2020characterizing, durieux2024empirical}, anti-patterns, and vulnerabilities, leading to compromised maintainability, file understandability, increased resource consumption, long build times, and reduced performance.


% \begin{itemize}
%     \item Complexity of Refactoring:

% Elaborate on the complexity of Dockerfile refactoring, including the potential impact on multiple instructions.
% Mention how each small change can introduce risks such as build failures, version mismatches, base image size issues, and environment variable misconfigurations.
% \end{itemize}
